Computationally efficient optimal control for unstable power system models

In this article, the focus is mainly on gaining the optimal control for the unstable power system models and stabilizing them through the Riccati-based feedback stabilization process with sparsity-preserving techniques. We are to find the solution of the Continuous-time Algebraic Riccati Equations (CAREs) governed from the unstable power system models derived from the Brazilian Inter-Connected Power System (BIPS) models, which are large-scale sparse index-1 descriptor systems. We propose the projection-based Rational Krylov Subspace Method (RKSM) for the iterative computation of the solution of the CAREs. The novelties of RKSM are sparsity-preserving computations and the implementation of time-convenient adaptive shift parameters. We modify the Low-Rank Cholesky-Factor integrated Alternating Direction Implicit (LRCF-ADI) technique based nested iterative Kleinman-Newton (KN) method to a sparse form and adjust this to solve the desired CAREs. We compare the results achieved by the Kleinman-Newton method with that of using the RKSM. The applicability and adaptability of the proposed techniques are justified numerically with MATLAB simulations. Transient behaviors of the target models are investigated for comparative analysis through the tabular and graphical approaches.

==> numcompress.tex <==
%%
%% This is file 'numcompress'.
%%
%% Copyright (C) 2009-2012 River Valley Technologies 
%%                    <latex.support@river-valley.com>
%%   
%% This package may be distributed under the terms of the LaTeX Project 
%% Public License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.0 or, at your option, any later version.
%%
%% $Id: numcompress.sty 187 2012-08-18 09:36:35Z rishi $
%% $URL: http://lenova.river-valley.com/svn/elsbst/trunk/numcompress.sty $
%%
\NeedsTeXFormat{LaTeX2e}
\def\Fileversion$#1: #2 ${\gdef\fileversion{#2}}
\def\Filedate$#1: #2-#3-#4 #5 #6 #7 ${\gdef\filedate{#2/#3/#4}} 
\Fileversion$Rev: 187 $
\Filedate$LastChangedDate: 2012-08-18 15:06:35 +0530 (Sat, 18 Aug 2012) $
\ProvidesPackage{numcompress}
   [\filedate\space\fileversion\space numcompress (CVR)]
\PackageWarningNoLine{numcompress}
   {****************************************\MessageBreak
    Package numcompress v,\fileversion\space loaded\MessageBreak
    [Compress numbers (CVR)]\MessageBreak
    ****************************************}
\newif\ifdots \dotsfalse
\newif\ifnumcompress \numcompresstrue

\DeclareOption{dots}{\global\dotstrue}
\DeclareOption{nodots}{\global\dotsfalse}
\DeclareOption{compress}{\global\numcompresstrue}
\DeclareOption{nocompress}{\global\numcompressfalse}

\ProcessOptions 

\def\removeDot#1{\def\tmp{#1}%
    \ifx\tmp\@empty\else\@removeDot#1\@nil\fi}

\def\@removeDot#1\@nil{\edef\fchar{\expandafter\@car#1\@nil}%
      \edef\rchar{\expandafter\@cdr#1!\@nil}%
      \def\@xmltempa{.}\def\@xmltempb{!}%
      \ifx\fchar\@xmltempb\relax\else%
      \ifx\fchar\@xmltempa\relax\else%
      \fchar\ignorespaces\fi\removeDot{\rchar}\fi}

\def\First[#1]{\csname First#1\endcsname}
\def\Second[#1]{\csname Second#1\endcsname}

\def\parseFirstPage#1{\@tempcnta=0
  \@tfor\@digits:=#1\do{%
    {\global\advance\@tempcnta by 1
      \expandafter\xdef\csname
      First\the\@tempcnta\endcsname{\@digits}%
      \xdef\flength{\the\@tempcnta}}}}

\def\parseSecondPage#1{\@tempcnta=0
  \@tfor\@digits:=#1\do{%
    {\global\advance\@tempcnta by 1
      \expandafter\xdef\csname
      Second\the\@tempcnta\endcsname{\@digits}%
      \xdef\llength{\the\@tempcnta}}}}

\newif\ifdissimilar\dissimilarfalse
\def\checkequal#1#2{\edef\Farg{#1}\edef\Sarg{#2}%
      \edef\One{A}%
      \ifcat\One\Farg \relax\else%
      \ifdissimilar\Sarg\else%
      \ifnum\Farg=\Sarg\relax\else\Sarg\dissimilartrue\fi\fi\fi}
%
\let\@@fpage\@empty
\let\@@lpage\@empty
\def\fpage@compress#1{%
      \gdef\@@fpage{#1}%
            \edef\llength{0}%
            \parseFirstPage{#1}%
      \ifnum\flength=\llength%
       \gdef\@fpage{\@@fpage}%
       \gdef\@lpage{%
        \@ifundefined{Second1}{}{\checkequal{\First[1]}{\Second[1]}}%
        \@ifundefined{Second2}{}{\checkequal{\First[2]}{\Second[2]}}%
        \@ifundefined{Second3}{}{\checkequal{\First[3]}{\Second[3]}}%
        \@ifundefined{Second4}{}{\checkequal{\First[4]}{\Second[4]}}%
        \@ifundefined{Second5}{}{\checkequal{\First[5]}{\Second[5]}}%
      }%
      \else%
       \gdef\@fpage{\@@fpage}%
       \gdef\@lpage{\@@lpage}%
     \fi}

\def\lpage@compress#1{%
        \gdef\@@lpage{#1}%
        \parseSecondPage{#1}%
      \ifnum\flength=\llength%
       \gdef\@fpage{\@@fpage}%
       \gdef\@lpage{%
       \edef\One{A}%
       \edef\xFirst{\First[1]}%
       \edef\xSecond{\Second[1]}%
       \ifcat\One\xSecond\relax%
          \ifx\xFirst\xSecond%
           \@ifundefined{Second1}{}{\checkequal{\First[1]}{\Second[1]}}%
           \@ifundefined{Second2}{}{\checkequal{\First[2]}{\Second[2]}}%
           \@ifundefined{Second3}{}{\checkequal{\First[3]}{\Second[3]}}%
           \@ifundefined{Second4}{}{\checkequal{\First[4]}{\Second[4]}}%
           \@ifundefined{Second5}{}{\checkequal{\First[5]}{\Second[5]}}%
          \else#1\fi%
      \else%
          \ifx\xFirst\xSecond%
           \@ifundefined{Second1}{}{\checkequal{\First[1]}{\Second[1]}}%
           \@ifundefined{Second2}{}{\checkequal{\First[2]}{\Second[2]}}%
           \@ifundefined{Second3}{}{\checkequal{\First[3]}{\Second[3]}}%
           \@ifundefined{Second4}{}{\checkequal{\First[4]}{\Second[4]}}%
           \@ifundefined{Second5}{}{\checkequal{\First[5]}{\Second[5]}}%
        \else#1\fi%
      \fi%
      }%
    \else
      \gdef\@fpage{\@@fpage}%
      \gdef\@lpage{%
      \edef\Targ{#1}%
      \edef\One{A}%
      \edef\xFirst{\First[1]}%
      \edef\xSecond{\Second[1]}%
      \ifx\xFirst\xSecond
         \ifcat\One\xSecond\relax\else\@@lpage\fi%
      \else#1\fi%
      }%
  \fi}

%\newwrite\xx
%\immediate\openout\xx=tmpbib.tex
\gdef\@@lpage@compress#1--#2\@nil{\lpage@compress{#1}}
\gdef\@@@pages#1#2{\def\next{#2}%
%  \immediate\write\xx{[\the\c@NAT@ctr.]\space [#1][#2]}%
  \fpage@compress{#1}%\ifx\next\@empty\relax\else
   \@@lpage@compress#2\@nil%\fi
  {\@fpage\ifx\next\@empty\relax\else
    --\@lpage\fi}\resetall}

\gdef\@@@page#1{#1\resetall}

\def\mk@empty#1{\@tempcnta=1
  \loop\ifnum\@tempcnta<6
    \expandafter\let\csname#1\the\@tempcnta\endcsname\relax
    \advance\@tempcnta by 1 \repeat}
\def\resetall{\let\@lpage\@empty\let\@fpage\@empty
   \def\flength{0}\def\llength{0}%
   \let\@@fpage\@empty\let\@@lpage\@empty
   \mk@empty{First}\mk@empty{Second}}


\ifdots
 \gdef\xfnm[#1]{\unskip\space#1}
 \def\bibinfo#1#2{\@ifnextchar.{\@@bibinfo{#1}{#2}}{\@@@bibinfo{#1}{#2}}}
 \def\@@@bibinfo#1#2{\def\next{#1}%
   \def\@@@pg{pages}\def\@@@au{author}%
   \ifx\next\@@@pg\bibpages{#2}\else
   \ifx\next\@@@au\bibauthor{#2}\else
   #2\fi\fi}
 \def\@@bibinfo#1#2.{\def\next{#1}%
  \def\@@@pg{pages}\def\@@@au{author}%
  \ifx\next\@@@pg\bibpages{#2}.\else
  \ifx\next\@@@au\bibauthor{#2}\else
  #2.\fi\fi}
\else
 \gdef\xfnm[#1]{\unskip\space\removeDot{#1}}
 \def\bibinfo#1#2{\def\next{#1}%
   \def\@@@pg{pages}\def\@@@au{author}%
   \ifx\next\@@@pg\bibpages{#2}\else
   \ifx\next\@@@au\bibauthor{#2}\else
   #2\fi\fi}
\fi

\ifnumcompress
 \def\bibpages#1{\@@bibpages#1--\\\@nil}
 \def\@@bibpages#1--#2\@nil{%
   \ifx\\#2\relax\@@@page{#1}\else
   \@@@pages{#1}{#2}\fi}
 \else
 \def\bibpages#1{#1}
\fi

\def\bibauthor#1{#1}

\endinput

%%
%% End of package 'numcompress.sty'
%%


==> preamble.tex <==
\usepackage[hardware,software]{mymacros}
%\usepackage{amsthm}
\usepackage{pgfplots}

\usepackage[vlined,longend,linesnumbered,ruled]{algorithm2e}
\providecommand{\dontprintsemicolon}{\DontPrintSemicolon}
\providecommand{\DontPrintSemicolon}{\dontprintsemicolon}
%\usepackage[colorlinks=true]{hyperref}

%\usepackage[list=true]{caption,subcaption} %list=true enables listing
                                %of subfigures in the list of figures
\usepackage{pgfplots}
\definecolor{mpiblue}{HTML}{006AA9}
\definecolor{mpigreen}{HTML}{5C871D}
\pgfplotscreateplotcyclelist{mylist1}{%
{black,solid},
{blue,dashed},
{mpigreen,dash pattern = on 3pt off 1pt on 1pt off 1pt},
{red,dash pattern = on 2pt off 2pt on 1pt off 2pt on 1pt off 2pt},
{cyan,densely dashed},
{mpiblue,densely dotted},
{magenta,dotted},
}
\usepackage{pgfplots}
\definecolor{mpiblue}{HTML}{006AA9}
\definecolor{mpigreen}{HTML}{5C871D}
\pgfplotscreateplotcyclelist{mylist1}{%
{black,solid},
{blue,dashed},
{mpigreen,dash pattern = on 3pt off 1pt on 1pt off 1pt},
{red,dash pattern = on 2pt off 2pt on 1pt off 2pt on 1pt off 2pt},
{cyan,densely dashed},
{mpiblue,densely dotted},
{magenta,dotted},
}
\pgfplotsset{every axis plot/.append style={line width=.75pt}}
% \DeclareMathOperator{\nul}{Null}
% \DeclareMathOperator{\rang}{Rang}
% \DeclareMathOperator{\Img}{Im}
% \DeclareMathOperator{\Rank}{rank}
% \DeclareMathOperator{\eps}{eps}
%\DeclareMathOperator{\Rel}{Re}
%\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\det}{de}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{remark}[theorem]{Remark}
\newcommand\norm[1]{\left\lVert#1\right\rVert}

% some help for emacs tex user
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main" 
%%% TeX-PDF-mode:t
%%% auto-fill-function:nil
%%% mode:auto-fill
%%% flyspell-mode:nil
%%% mode:flyspell
%%% ispell-local-dictionary: "en_US"
%%% End: 
     



==> primble.tex <==
\usepackage[hardware,software]{latexmacros/mymacros}
\usepackage{amsthm}
\usepackage{pgfplots}

\usepackage[vlined,longend,linesnumbered,ruled]{algorithm2e}
\providecommand{\dontprintsemicolon}{\DontPrintSemicolon}
\providecommand{\DontPrintSemicolon}{\dontprintsemicolon}
%\usepackage[colorlinks=true]{hyperref}

\usepackage[list=true]{caption,subcaption} %list=true enables listing
                                %of subfigures in the list of figures
\usepackage{pgfplots}
\definecolor{mpiblue}{HTML}{006AA9}
\definecolor{mpigreen}{HTML}{5C871D}
\pgfplotscreateplotcyclelist{mylist1}{%
{black,solid},
{blue,dashed},
{mpigreen,dash pattern = on 3pt off 1pt on 1pt off 1pt},
{red,dash pattern = on 2pt off 2pt on 1pt off 2pt on 1pt off 2pt},
{cyan,densely dashed},
{mpiblue,densely dotted},
{magenta,dotted},
}
\usepackage{pgfplots}
\definecolor{mpiblue}{HTML}{006AA9}
\definecolor{mpigreen}{HTML}{5C871D}
\pgfplotscreateplotcyclelist{mylist1}{%
{black,solid},
{blue,dashed},
{mpigreen,dash pattern = on 3pt off 1pt on 1pt off 1pt},
{red,dash pattern = on 2pt off 2pt on 1pt off 2pt on 1pt off 2pt},
{cyan,densely dashed},
{mpiblue,densely dotted},
{magenta,dotted},
}
\pgfplotsset{every axis plot/.append style={line width=.75pt}}
\DeclareMathOperator{\nul}{Null}
\DeclareMathOperator{\rang}{Rang}
\DeclareMathOperator{\Rel}{Re}
\DeclareMathOperator{\Img}{Im}
\DeclareMathOperator{\Rank}{rank}
\DeclareMathOperator{\eps}{eps}
\DeclareMathOperator{\Rel}{Re}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\det}{det}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newcommand\norm[1]{\left\lVert#1\right\rVert}

% some help for emacs tex user
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main" 
%%% TeX-PDF-mode:t
%%% auto-fill-function:nil
%%% mode:auto-fill
%%% flyspell-mode:nil
%%% mode:flyspell
%%% ispell-local-dictionary: "en_US"
%%% End: 
     


